Retrieval-Augmented LLM Agents: Learning to Learn from Experience

While large language models (LLMs) have advanced the development of general-purpose agents, robust generalization to unseen tasks remains challenging. Two common approaches are supervised fine-tuning and training-free memory-augmented generation using retrieved experience; yet both have limitations: fine-tuning often fails to extrapolate to new tasks, while experience retrieval often underperforms compared to supervised baselines. In this work, we combine these approaches and study how retrieval-augmented LLM agents can learn to use retrieved trajectories in-context. First, we establish a strong LoRA fine-tuning baseline that outperforms several state-of-the-art agent training pipelines. Second, we analyze key design choices for experience retrieval, including storage, querying, and trajectory selection. We then integrate experience retrieval directly into the fine-tuning process, finding that this substantially improves generalization to unseen tasks. Finally, we show that these gains often persist with imperfect experience and, even when agents reuse their own failed attempts without test-time parameter updates. Overall, our results establish simple episodic retrieval as a strong foundation for agent memory and retrieval-aware fine-tuning as a practical and effective framework for building agents that learn to learn from experience.

==> macros.tex <==
\ProvidesFile{macros.tex}[2026/08/26 Reusable paper macros]

\RequirePackage{xparse}
\RequirePackage{etoolbox}
\setlength{\marginparwidth}{2cm}
\RequirePackage[textsize=tiny]{todonotes}


\newcommand{\PaperVersionName}{}
\newif\ifaclversion
\newif\ifarxivversion
\aclversionfalse
\arxivversionfalse

\NewDocumentCommand{\SetPaperVersion}{m}{%
  \renewcommand{\PaperVersionName}{#1}%
  \ifdefstring{#1}{acl}{\aclversiontrue}{\aclversionfalse}%
  \ifdefstring{#1}{arxiv}{\arxivversiontrue}{\arxivversionfalse}%
}

\newcommand{\PaperVersionNotSetError}{%
  \PackageError{paper-template}
    {No paper version has been selected}
    {Call \string\SetPaperVersion\{name\} in the active main file.}%
}

\NewDocumentCommand{\IfPaperVersionTF}{m +m +m}{%
  \ifdefempty{\PaperVersionName}
    {\PaperVersionNotSetError}
    {\ifdefstring{\PaperVersionName}{#1}{#2}{#3}}%
}

\NewDocumentCommand{\OnlyPaperVersion}{m +m}{%
  \IfPaperVersionTF{#1}{#2}{}%
}

\NewDocumentCommand{\PaperVersionTwo}{m +m m +m}{%
  \IfPaperVersionTF{#1}
    {#2}
    {\IfPaperVersionTF{#3}
      {#4}
      {\PackageError{paper-template}
        {Paper version `\PaperVersionName' is not supported here}
        {Select either `#1' or `#3', or update this \string\PaperVersionTwo\space call.}}}%
}

\NewDocumentCommand{\PaperVersionThree}{m +m m +m m +m}{%
  \IfPaperVersionTF{#1}
    {#2}
    {\IfPaperVersionTF{#3}
      {#4}
      {\IfPaperVersionTF{#5}
        {#6}
        {\PackageError{paper-template}
          {Paper version `\PaperVersionName' is not supported here}
          {Select `#1', `#3', or `#5', or update this \string\PaperVersionThree\space call.}}}}%
}

\NewDocumentCommand{\ACLorOther}{+m +m}{\IfPaperVersionTF{acl}{#1}{#2}}
\NewDocumentCommand{\ArxivOrOther}{+m +m}{\IfPaperVersionTF{arxiv}{#1}{#2}}
\NewDocumentCommand{\ACLorArxivorOther}{+m +m +m}{%
  \PaperVersionThree{acl}{#1}{arxiv}{#2}{iclr}{#3}%
}
\NewDocumentCommand{\OnlyACL}{+m}{\OnlyPaperVersion{acl}{#1}}
\NewDocumentCommand{\OnlyArxiv}{+m}{\OnlyPaperVersion{arxiv}{#1}}
\NewDocumentCommand{\NotACL}{+m}{\IfPaperVersionTF{acl}{}{#1}}
\NewDocumentCommand{\NotArxiv}{+m}{\IfPaperVersionTF{arxiv}{}{#1}}


\providecommand{\paragraphshortstyle}[1]{\paragraph{#1}}
\NewDocumentCommand{\paragraphshort}{m}{\paragraphshortstyle{#1}}


\newif\ifPaperTodos
\PaperTodostrue

\newcommand{\ShowPaperTodos}{\PaperTodostrue}
\newcommand{\HidePaperTodos}{\PaperTodosfalse}

\NewDocumentCommand{\PaperTodo}{O{} m m +m}{%
  \ifPaperTodos
    \todo[inline,author={#2},color={#3},size=\scriptsize,caption={},#1]{#4}%
  \fi
}

\NewDocumentCommand{\PaperMarginTodo}{O{} m m +m}{%
  \ifPaperTodos
    \todo[author={#2},color={#3},size=\scriptsize,fancyline,caption={},#1]{#4}%
  \fi
}

\NewDocumentCommand{\thomas}{O{} +m}{%
  \PaperTodo[#1]{Thomas}{green!30}{#2}%
}

\NewDocumentCommand{\thomasmargin}{O{} +m}{%
  \PaperMarginTodo[#1]{Thomas}{green!30}{#2}%
}

